Comparison of the O(3) Bootstrap $\sigma$-Model with the Lattice Regularization at Low Energies

The renormalized coupling $\gr$ defined through the connected 4-point function at zero external momentum in the non-linear O(3) sigma-model in two dimensions, is computed in the continuum form factor bootstrap approach with estimated error $\sim 0.3%$. New high precision data are presented for $\gr$ in the lattice regularized theory with standard action for nearly thermodynamic lattices $L/\xi\sim 7$ and correlation lengths $\xi$ up to $\sim 122$ and with the fixed point action for correlation lengths up to $\sim 12$. The agreement between the form factor and lattice results is within $\sim 1%$. We also recompute the phase shifts at low energy by measuring the two-particle energies at finite volume, a task which was previously performed by L\"uscher and Wolff using the standard action, but this time using the fixed point action. Excellent agreement with the Zamolodchikov S-matrix is found.

==> sect2 <==
%\section{Definitions}
\subsection{Definitions}

Consider a general continuum quantum field theory in 
two dimensions, in infinite volume, 
with global O($n$) symmetry. 
Let $\sigma^a(x)$, $a=1\dots n$ be a vector multiplet of (renormalized) 
Euclidean scalar fields with 2-point function
\begin{equation}
S^{a_1a_2}(x_1,x_2)=\langle \sigma^{a_1}(x_1)\sigma^{a_2}(x_2) \rangle\,. 
\end{equation}
The inverse of its Fourier transform  
\begin{equation}
\label{twopoint}
G(k)\delta^{a_1a_2}=\int \rmd^2 x e^{ikx} S^{a_1a_2}(x,0)\,,
\end{equation}
is assumed to have an expansion for small momenta
\begin{equation}
G(k)^{-1}=\Zr^{-1}\Big( \Mr^2 + k^2 +O(k^4)\Bigr)\,.
\label{nxi1}
\end{equation}

We denote the 4-point function by
\begin{equation}   
S^{a_1a_2a_3a_4}(x_1,x_2,x_3,x_4)=
\langle
\sigma^{a_1}(x_1)\sigma^{a_2}(x_2)\sigma^{a_3}(x_3)\sigma^{a_4}(x_4)
\rangle\,,
\end{equation}
and the connected 4-point function
\begin{eqnarray}
&S_c^{a_1a_2a_3a_4}(x_1,x_2,x_3,x_4)=S^{a_1a_2a_3a_4}(x_1,x_2,x_3,x_4)
-S^{a_1a_2}(x_1,x_2)S^{a_3a_4}(x_3,x_4)
\nonumber
\\
&
-S^{a_1a_3}(x_1,x_3)S^{a_2a_4}(x_2,x_4)
-S^{a_1a_4}(x_1,x_4)S^{a_2a_3}(x_2,x_3).
\end{eqnarray}
Introducing the Fourier transform by
\begin{equation}
\widetilde{S}^{a_1a_2a_3a_4}(k_1,k_2,k_3,k_4)=\int\prod_{j=1}^4
\left[ \rmd^2 x_j e^{ik_jx_j}\right]
S^{a_1a_2a_3a_4}(x_1,x_2,x_3,x_4)\,,
\end{equation}
and similarly $\widetilde{S}_c$ for the connected part,
the conventional zero momentum (dimensionless) coupling (in two
dimensions) is defined by
\begin{equation}
\gr= -{\Mr^2\over G(0)^2}
{1\over n^2}\sum_{a,b}G^{aabb}(0,0,0,0)\,,
\end{equation}
where
\begin{equation}
\widetilde{S}_c^{a_1a_2a_3a_4}(k_1,k_2,k_3,k_4)
=(2\pi)^2\delta^{(2)}(k_1+k_2+k_3+k_4)G^{a_1a_2a_3a_4}(k_1,k_2,k_3,k_4)\,.
\end{equation}

We will assume that the 2-point function has a spectral representation
\begin{equation}
\label{specrep}
G(k)=Z\int_0^{\infty} \rmd\mu {\rho(\mu)\over \mu^2 +k^2}\,,
\end{equation}
where the normalization constant $Z$ takes into account that,
assuming that the spectrum of the theory 
contains a vector multiplet of stable particles of mass $M$,
we normalize the spectral density $\rho$ 
so that the 1-particle contribution is
\begin{equation}
\rho^{(1)}(\mu)=\delta(\mu-M).
\end{equation}
Then the coefficients appearing in the small momenta expansion above
can be expressed as
\begin{equation}
\Zr=Z{\gamma_2^2\over\delta_2}\,,
\end{equation}
\begin{equation}
{\Mr^2\over M^2}={\gamma_2\over\delta_2}\,,  
\label{nxi2}
\end{equation}
where $\gamma_2$ and $\delta_2$ are the moments
\begin{gather}
\gamma_2=M^2\int \rmd \mu \,{\rho(\mu)\over\mu^2},
\\
\delta_2=M^4\int \rmd \mu \,{\rho(\mu)\over\mu^4}\,.
\end{gather}

Further the coupling $\gr$ can be written as
\begin{equation}
\gr=-{n+2\over n} {\gamma_4\over \gamma_2\delta_2}
\end{equation}
where $\gamma_4$ is defined through
\begin{equation}
G^{a_1a_2a_3a_4}(0,0,0,0)={Z^2\gamma_4\over M^6}
\left( 
 \delta^{a_1a_2}\delta^{a_3a_4}
+\delta^{a_1a_3}\delta^{a_2a_4}
+\delta^{a_1a_4}\delta^{a_2a_3}\right)\,.
\end{equation}

Strictly speaking, all observable physics (in a massive theory) 
is on-shell; different interpolating fields give the same results.
Off-shell amplitudes 
of particular composite (and `elementary') 
operators, are only of physical interest
if they are sources of (idealized) infinitesimal weakly 
interacting probes.
The fields are characterized by their various 
quantum numbers and their dimensions e.g. coded
in the behavior of the 2-point function $G(k)$.
The assumption eq.(\ref{specrep}) corresponds to a limitation
on the behavior of the associated spectral function
$\rho(\mu)$ as $\mu\to\infty$.
It is an implicit connection to the
association of $\sigma^a(x)$ with a particular local field in the
Lagrangian quantum field theory.  
In the non-linear $O(n)$ sigma model the \lq elementary' field
$\sigma^a(x)$ is characterized by its vanishing engineering dimension
(in addition to being an isovector and spacetime scalar).
We can therefore assume that the short distance singularities of its
two-point function are sufficiently weak (only logarithmic) so that
the spectral representation (\ref{specrep}) holds without subtractions.
Indeed, in the FFB approach, this uniquely defines (up to normalization)
an operator $\hat\sigma^a(x)$, which has form factors that are not
growing too fast at infinity so that the corresponding spectral
density $\rho(\mu)$ vanishes fast enough for $\mu\to\infty$.

%{\bf Should we mention the Usual definition of an on-shell $\gr$ from
%the S-matrix???}


%\vfill
%\eject








